Projected Density Matrix Sampling for Lattice Hamiltonians

Quantum Monte Carlo methods are powerful tools for studying quantum many-body systems but face difficulties in accessing excited states and in treating sign problems. We present a continuous-time path-integral Monte Carlo method for computing the low-lying spectrum of generic quantum Hamiltonians within a projection subspace. The method projects the thermal density matrix onto a subspace spanned by a chosen set of linearly independent states. It is free of Trotter discretization errors and systematically converges to the low-energy states which have finite overlap with the projection subspace as the $\beta$ parameter increases. While most effective for systems without a sign problem, the method also yields information about low-energy spectra when sign problems are present. We illustrate the approach on two problems. For the sign-free case, we compute the first four low-energy levels in the scaling limit of the one-dimensional Ising model with both transverse and longitudinal fields, demonstrating the flow from the conformal limit to the massive $E_8$ quantum field theory. For the sign-problem case, we apply the method to the frustrated Shastry-Sutherland model and benchmark it against exact diagonalization on small lattices. We also present results for larger systems beyond the lattice sizes accessible to exact diagonalization, while limited to small $\beta$ where sign problems occur. Our method provides a general route toward quantum Monte Carlo spectroscopy for lattice Hamiltonians.

==> header-1.tex <==
\ifx\pdfsuppresswarningpagegroup\undefined\else\pdfsuppresswarningpagegroup=1\fi\relax
\RequirePackage{silence}
% We know this warning: Revtex does change \label, but fixes it for nameref as well
\WarningFilter{nameref}{The definition of \label has changed!}
% revtex will change the float package, OK, we are warned
\WarningFilter{revtex4-2}{Repair the float package}

\AtBeginDocument{\RenewCommandCopy\qty\SI}

\PassOptionsToPackage{unicode, pdfprintscaling=None, colorlinks}{hyperref}
% The curious construction is to unconfuse overleaf: it is simply the \documentclass command
%\expandafter\relax\csname documentclass\endcsname[aps,prx,reprint,nofootinbib,preprintnumbers,floatfix,unsortedaddress,superscriptaddress,longbibliography]{revtex4-2}

\usepackage{orcidlink,multirow,colortbl,dcolumn,ulem,tikz,graphicx,latexsym,amsmath,amssymb,amsfonts,bm,bbm,microtype,xspace,placeins,float,mathtools,xcolor,makecell,tabularx, booktabs, longtable, supertabular, hyperref, array}

\usepackage[export]{adjustbox}
\usepackage[capitalise]{cleveref}

% siunitx / physics setup
\usepackage{siunitx}
\usepackage{physics}

% Suppress the siunitx warning about physics package
\ExplSyntaxOn
\msg_redirect_name:nnn{siunitx}{physics-pkg}{none}
\ExplSyntaxOff

% Restore \qty to siunitx version
\AtBeginDocument{\RenewCommandCopy\qty\SI}




% -------------------------------------------

\usetikzlibrary{decorations.markings, arrows, decorations.pathmorphing}
\graphicspath{{pic/}}
\allowdisplaybreaks
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newlength{\FigureWidth}
\setlength{\FigureWidth}{3.3in}
\newlength{\RowHeight}
\setlength{\RowHeight}{1.5em}
\newcolumntype{L}[1]{>{\raggedright\arraybackslash\rule{0pt}{\RowHeight}}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash\rule{0pt}{\RowHeight}}p{#1}}
\newcolumntype{R}[1]{>{\raggedleft\arraybackslash\rule{0pt}{\RowHeight}}p{#1}}
\newcolumntype{M}[1]{>{\centering\arraybackslash\rule{0pt}{\RowHeight}}m{#1}}
\newcommand\TopRule{\Xhline{0.08em}}
\newcommand\HeaderRule{\Xhline{0.05em}}
\newcommand\MidRule{\Xhline{0.03em}}
\newcommand\BotRule{\Xhline{0.08em}}
\newcommand\SetTableProperties{
  \renewcommand{\arraystretch}{1.4}
}

\makeatletter
\newcommand\showtitleinbib{{\escapechar=`\\ \immediate\write\@auxout{%
\csname citation{REVTEX42Control}\endcsname^^J%
\csname citation{apsrev42Control}\endcsname
}}}
\makeatother

